On Simultaneous Long-Short Stock Trading Controllers with Cross-Coupling

The Simultaneous Long-Short(SLS) controller for trading a single stock is known to guarantee positive expected value of the resulting gain-loss function with respect to a large class of stock price dynamics. In the literature, this is known as the Robust Positive Expectation(RPE)property. An obvious way to extend this theory to the trading of two stocks is to trade each one of them using its own independent SLS controller. Motivated by the fact that such a scheme does not exploit any correlation between the two stocks, we study the case when the relative sign between the drifts of the two stocks is known. The main contributions of this paper are three-fold: First, we put forward a novel architecture in which we cross-couple two SLS controllers for the two-stock case. Second, we derive a closed-form expression for the expected value of the gain-loss function. Third, we use this closed-form expression to prove that the RPE property is guaranteed with respect to a large class of stock-price dynamics. When more information over and above the relative sign is assumed, additional benefits of the new architecture are seen. For example, when bounds or precise values for the means and covariances of the stock returns are included in the model, numerical simulations suggest that our new controller can achieve lower trading risk than a pair of decoupled SLS controllers for the same level of expected trading gain.

==> README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de


==> gainlossdynamics.tex <==
{
We can readily see from Section \ref{sec:egformula} that \m{\Exp{g(N)}} is linearly proportional to the values of \m{I_{_{01}}} and \m{I_{_{02}}}, irrespective of the values of \m{|\mu_1|} and \m{|\mu_2|} or the other parameters.
For fixed values of the CC-SLS controller design parameters, as the trading frequency increases, the magnitude of the mean price returns \m{|\mu_1|} and \m{|\mu_2|} of the two stocks decreases.
Here we obtain some insights into \m{\Exp{g(N)}} when either the feedback parameters or the mean price returns are small enough such that \m{K_1|\mu_1|\ll 1} and \m{K_2|\mu_2|\ll 1}.
\\[\gap]
{\bf Proposition:} \emph{
For two stocks with stochastically varying prices having mean returns \m{\mu_1\neq 0} and \m{\mu_2\neq 0} respectively being traded by 2-SLS and CC-SLS controller designs having \m{K_1|\mu_1|\ll 1} and \m{K_2|\mu_2|\ll 1}, the expected values of their respective trading gain-loss functions at stage \m{N} can be approximated as
\begin{align*}
 \Exp{g(N)} &\approx N(N-1) \Bigl[I_{_{01}}K_1\mu_1 (\mu_1 +\coupling \mu_2)\\ &\hspace{3cm}+ I_{_{02}}K_2\mu_2 (\mu_2 + \coupling \mu_1)\Bigl].
\end{align*}
}\\[-10pt]
{\bf Proof:}
The linear approximation of \m{\phi_N(x)} for \m{|x|\ll 1} can be obtained using
\begin{align*}
 \phi_N(x) = (1 + x)^N+ (1 - x)^N-2\approx N(N-1)x^2.
\end{align*}
Assuming \m{K_1|\mu_1|\ll 1} and \m{K_2|\mu_2|\ll 1} leads to 
$$
\theta\ll 1;\;\; |\alpha_1|\ll 1;\;\; |\alpha_2|\ll 1;\;\; |\beta_1|\ll 1;\;\; |\beta_2|\ll 1.
$$
Using the above in conjunction with the linear approximation of \m{\phi_N(x)} for \m{|x|\ll 1} in the expression for \m{\Exp{g(N)}} above and simplifying, we get
\if 0
\begin{gather*}
\Exp{g(N)} 
\approx
\frac{N(N-1)}{2\theta}\Bigl[
 2\coupling \mu_1\mu_2  (I_{_{01}}K_1+ I_{_{02}}K_2) (\alpha_1
+\alpha_2)\\+\alpha_1\cdot (I_{_{02}}\mu_2\beta_1 + I_{_{01}}\mu_1\beta_2)
+ \alpha_2\cdot (I_{_{02}}\mu_2\beta_2 + I_{_{01}}\mu_1\beta_1)
 \Bigl].
\end{gather*}
Further simplification and rearrangement of the terms above yields
\fi
\begin{align*}
\Exp{g(N)} 
&\approx
\frac{N(N-1)}{2\theta}\Bigl[
 2\coupling \mu_1\mu_2  (I_{_{01}}K_1+ I_{_{02}}K_2) \theta\\
&+I_{_{02}}\mu_2\cdot (\alpha_1\beta_1 + \alpha_2\beta_2)
+ I_{_{01}}\mu_1\cdot (\alpha_1\beta_2 + \alpha_2\beta_1)
 \Bigl].
\end{align*}
Now,
\begin{align*}
 \alpha_1\beta_1+\alpha_2\beta_2 
&= 2K_2\mu_2\theta;\\[\gap]
 \alpha_1\beta_2+\alpha_2\beta_1 &= 2K_1\mu_1\theta.
 \end{align*}
 Substituting these, we get 
 \begin{align*}
\Exp{g(N)} 
&\approx
{N(N-1)}\Bigl[
 \coupling \mu_1\mu_2  (I_{_{01}}K_1+ I_{_{02}}K_2) \\
&\hspace{3cm}+I_{_{02}}K_2\mu_2^2
+ I_{_{01}}K_1\mu_1^2
 \Bigl]\\
 &={N(N-1)}\Bigl[
 I_{_{01}}K_1\mu_1(\mu_1+\coupling\mu_2)\\
&\hspace{3cm} + I_{_{02}}K_2\mu_2(\mu_2+\coupling\mu_1)
 \Bigl]. \qed
\end{align*}
{\bf Remarks:} This result reveals that \m{\Exp{g(N)}} is approximately linearly proportional to \m{I_{0i}K_i} for \m{i=1,2} for small values of \m{K_1|\mu_1|} and \m{K_2|\mu_2|}. That is, in this operating range, the individual values of \m{I_{0i}} and \m{K_i} are irrelevant to the value of \m{\Exp{g(N)}} as long as the product \m{I_{0i}K_i} remains a constant. As a result, the trader has access to effectively fewer design choices with respect to controlling the expected trading gains in this operating range than indicated by the number of parameters.
In addition, we see that \m{\Exp{g(N)}} is approximately linearly proportional to the coupling coefficient \m{\coupling}.
Finally, \m{\Exp{g(N)}} is approximately quadratic in \m{\mu_1}, \m{\mu_2} and \m{N}.}


==> nonLinearSetup.tex <==
The trading setup with nonlinear feedback is illustrated in Figure~\ref{nlsetup}.
We consider a stock having stochastically varying price~$S(k)$ beginning at \m{S(0)>0} which is known. 
The underlying returns 
$$
\rho(k)\doteq \frac{S(k+1)-S(k)}{S(k)}
$$ 
are assumed to be independent and identically distributed random variables, each with unknown probability density function~$h$ that is piecewise continuous, symmetric with respect to its mean \m{\mu_{_h}} and nonincreasing to the right of \m{\mu_{_h}}. Note that symmetry forces \m{h} to be nondecreasing to the left of \m{\mu_{h}}.
In the sequel, we take \m{\mathcal{H}} to be the collection of all such density functions and seek robust positivity of the expected cumulative trading gain-loss function \m{g(k)} with respect to \m{h\in\mathcal{H}}. \\[5pt]
{\bf Remark:} Note that \m{h\in\mathcal{H}} being nondecreasing to the left of \m{\mu_{_h}} and nonincreasing to its right results in the corresponding cumulative distribution function being convex to the left of \m{\mu_{_h}} and concave to the right. This is the description for unimodal distributions in~\cite{wintner1938asymptotic}, which leads to results along the lines central to the proof of our theorem to follow, and further pursued in papers such as~\cite{dharmadhikari1988unimodality} and~\cite{purkayastha1998simple}.
\begin{figure}[!ht]
\centering
\includegraphics [width=3.5in, trim={1cm 0 0 0},clip]{chap4f/NonlinearFeedback.pdf}
\caption{Trading Setup with Nonlinear Feedback}
\label{nlsetup}
\vspace{-0.0em}\end{figure}
\paragraph{Investments Using Price Trends:}
The investment level \m{I(k)} in the stock at stage~$k$ is obtained via nonlinear feedback. That is, 
\begin{align*}
I(k) &= f(x(k))
\end{align*}
where \m{x(k)} is a {\it trend indicator} of the price dynamics with initial value \m{x(0)=0} and is taken to be a weighted sum of the past returns. That is, for \m{k>0},
$$
x(k) \doteq
             \sum_{i=0}^{k-1} w_k(i)\rho(i).
$$
where \m{w_k(i)} are nonnegative weights, not all zero, used by the trader.
Note that mean return \m{\mu_{_h}} for each \m{\rho(i)} enforces
$$
\Exph{x(k)}=\mu_h \sum_{i=0}^{k-1} w_k(i),
$$
where the subscript \m{h} is used to emphasize expectation with respect to the unknown distribution of the returns.
\paragraph{Gain-Loss Function and Account Value:}
For the closed loop system with \m{g(0)=0}, 
we have
\begin{align*}
g(k+1) &= g(k) + I(k)\rho(k)\\
&= g(k) + f(x(k))\rho(k)
\end{align*}
with resulting account value~$V(k)$,
under assumption of zero risk-free rate of return, obtained as
$$
V(k) = V(0) + g(k)
$$
with initial value~$V(0)>0$. 
\paragraph{Nonlinear Feedback Control:}
The investment function \m{f:\real\to\real} is continuous and taken to be such that \m{f(x)>0} for all \m{x>0} and \m{f(-x)=-f(x)} for all \m{x\in\real}. 
Thus, a positive trend indicator \m{x(k)} leads to \m{f(x(k))>0}, which implies that the trader is \emph{long} on the stock. Similarly, a negative \m{x(k)} leads to the trader being \emph{short} on the stock. Enforcing \m{f(-x)=-f(x)} reflects the trader's indifference to the sign of market trend indicator.
In the sequel, we use \m{\mathcal{F}} to denote this class of nonlinear functions and note that it includes linear functions as a special case.
\paragraph{Example:}
Figure~\ref{samplepath} illustrates the internal working of the above trading setup using a simple example of investment using nonlinear feedback. For \m{252} stages, we trade a single sample path of stock price \m{S(k)} with returns obtained from a truncated normal distribution with mean \m{\mu = 0.0023} and standard deviation \m{\sigma=0.035} such that the deviation \m{|\rho(k)-\mu|\leq 0.075}.
The trend indicator \m{x(k)} is obtained as 
$$
x(k) = \begin{cases}
        \hspace{.2cm}\displaystyle\sum_{i=0}^{k-1} \rho(i)\;\;\; &\text{ for } k < 15;\\
        \\
        \displaystyle\sum_{i=k-15}^{k-1}\hspace{-0.2cm} \rho(i)\;\;\; &\text{ for } k \geq 15,
       \end{cases}
$$
with the investment level \m{I(k) = f(x(k))} in the stock obtained using the saturated linear function
$$
f(x) = \begin{cases}
        \min\{10 x, I_{sat}\} &\text{ for } x>0;\\
        \max\{10 x, -I_{sat}\} &\text{ for } x\leq 0,
       \end{cases}
$$
where \m{I_{sat}=2.} In the figure, the stages where the investment level is obtained from the linear part of \m{f(x(k))} are depicted in black, whereas saturation of the investment function is highlighted in red.
The last panel of the figure represents the gain-loss function \m{g(k)} for this sample path.
\begin{figure}[!h]
\centering
 \includegraphics[trim={1cm 0 0 0, clip}, width=5in]{chap4f/Nonlinear_Working_2_by_2.png}
 \vspace{-.75cm}
 \caption{Simple Example with Saturated Linear Investment Function}
 \label{samplepath}
\end{figure}
\medskip

